DeCoRe: Decoding by Contrasting Retrieval Heads to Mitigate Hallucinations

Large Language Models (LLMs) often hallucinate, producing unfaithful or factually incorrect outputs by misrepresenting the provided context or incorrectly recalling internal knowledge. Recent studies have identified specific attention heads within the Transformer architecture, known as retrieval heads, responsible for extracting relevant contextual information. We hypothesise that masking these retrieval heads can induce hallucinations and that contrasting the outputs of the base LLM and the masked LLM can reduce hallucinations. To this end, we propose Decoding by Contrasting Retrieval Heads (DeCoRe), a novel training-free decoding strategy that amplifies information found in the context and model parameters. DeCoRe mitigates potentially hallucinated responses by dynamically contrasting the outputs of the base LLM and the masked LLM, using conditional entropy as a guide. Our extensive experiments confirm that DeCoRe significantly improves performance on tasks requiring high contextual faithfulness, such as summarisation (XSum by 18.6%), instruction following (MemoTrap by 10.9%), and open-book question answering (NQ-Open by 2.4% and NQ-Swap by 5.5%).

==> figures/musique_entropy.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{assets/musique_closed_book_llama3_8b_instruct_decore_entropy_alpha_all_generation_step.pdf}
        \caption{Closed Book.}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{assets/musique_open_book_llama3_8b_instruct_decore_entropy_alpha_all_generation_step.pdf}
        \caption{Open Book.}
    \end{subfigure}
    \caption{Conditional Entropy over time in the MuSiQue task with CoT reasoning.}
    \label{fig:musique_decore_entropy_alpha_generation_step}
\end{figure}

==> figures/task_categorisation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.75\textwidth]{assets/Task_Categorisation.pdf}
    \caption{Tasks Categorisation}
    \label{fig:task_categories}
\end{figure}

==> figures/xsum_truthfulqa_entropy.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{assets/xsum_llama3_8b_instruct_decore_entropy_alpha_generation_step.pdf}
        \caption{XSum.}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{assets/truthfulqa_llama3_8b_instruct_decore_entropy_alpha_generation_step.pdf}
        \caption{TruthfulQA.}
    \end{subfigure}
    \caption{Entropy over time in the XSum and TruthfulQA tasks.}
    \label{fig:xsum_truthfulqa_decore_entropy_alpha_generation_step}
\end{figure}

==> tables/result_ablation_entropy_factuality.tex <==
\begin{table}
    \centering
    \caption{Ablation study of the upper limit of entropy $\text{max}_{\alpha}$ in the factuality tasks.}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lccccccc}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{TruthfulQA (MC)}} & \textbf{TriviaQA} & \textbf{PopQA} & \multicolumn{2}{c}{\textbf{NQ}} \\
        \cmidrule(lr){2-4}
        \cmidrule(lr){5-5}
        \cmidrule(lr){6-6}
        \cmidrule(lr){7-8}
                                        & \textbf{MC1 $\uparrow$} & \textbf{MC2 $\uparrow$} & \textbf{MC3 $\uparrow$} & \textbf{EM $\uparrow$} &  \textbf{EM $\uparrow$} & \textbf{Open $\uparrow$} & \textbf{Closed $\uparrow$} \\
        \midrule
        Llama3-8b-Instruct          & 39.29 & 55.66 & 30.16 & 53.46 & 21.10 & 69.72 & 29.19 \\
        + DeCoRe entropy (Ours)     & 36.97 & 54.33 & 28.93 & 56.36 & 24.54 & 70.06 & 28.47 \\
        + ($\text{max}_\alpha=0.5$) & 38.68 & 54.55 & 29.16 & 56.93 & 23.24 & 70.47 & 29.15 \\
        + ($\text{max}_\alpha=1$)   & 37.21 & 54.36 & 28.44 & 56.91 & 24.67 & 70.21 & 28.89 \\
        + ($\text{max}_\alpha=2$)   & 36.84 & 54.22 & 28.53 & 56.71 & 24.81 & 70.06 & 28.70 \\
        + ($\text{max}_\alpha=4$)   & 36.97 & 54.34 & 28.96 & 56.37 & 24.60 & 70.06 & 28.48 \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:result_ablation_entropy_factuality}
\end{table}

==> tables/result_ablation_entropy_faithfulness.tex <==
\begin{table}
    \centering
    \caption{Ablation study of the upper limit of entropy $\text{max}_{\alpha}$ in the faithfulness tasks.}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lcccccc}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{XSum}} & \multicolumn{2}{c}{\textbf{MemoTrap}} & \textbf{NQ-Swap} \\
        \cmidrule(lr){2-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-7}
                                        & \textbf{ROUGE-L $\uparrow$} & \textbf{BERTScore-F1 $\uparrow$} & \textbf{factKB $\uparrow$} & \textbf{Macro Acc $\uparrow$} & \textbf{Micro Acc $\uparrow$} & \textbf{EM $\uparrow$} \\
        \midrule
        Llama3-8b-Instruct          & 20.00 & 67.04 & 44.57 & 65.89 & 64.44 & 60.91 \\
        + DeCoRe entropy            & 19.60 & 67.21 & 57.37 & 69.39 & 68.37 & 65.87 \\
        + ($\text{max}_\alpha=0.5$) & 19.78 & 67.31 & 52.71 & 66.91 & 64.71 & 63.61 \\
        + ($\text{max}_\alpha=1$)   & 19.64 & 67.24 & 55.59 & 66.07 & 64.16 & 64.94 \\
        + ($\text{max}_\alpha=2$)   & 19.60 & 67.23 & 57.26 & 68.48 & 67.23 & 65.87 \\
        + ($\text{max}_\alpha=4$)   & 19.60 & 67.21 & 57.37 & 69.49 & 68.49 & 65.87 \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:result_ablation_entropy_faithfulness}
\end{table}



